Representation and Model Contributions on Small Molecular Benchmarks: Controlled Comparisons and External Evaluation

Improvements in molecular property prediction are usually attributed to the model, although part of the gain may come from the molecular representation. New models are commonly benchmarked against a random forest (RF) trained on a molecular fingerprint, a comparison that changes the model and the representation at the same time. We separate the two contributions with a two-by-two factorial design in which the RF and a second model (CatBoost or the tabular foundation models TabPFN and TabFM) are each trained on a fingerprint and on RDKit descriptors, and each effect is tested with a paired scaffold bootstrap. Seven small MoleculeNet datasets (3 regression, 4 classification) are evaluated on the published split of a recent graph transformer (DGT), on 10 additional scaffold splits and on external datasets. For solubility and lipophilicity, the representation effect exceeds the model effect in every main factorial design, in all three evaluations. For hydration free energy, the result depends on the starting fingerprint: from ECFP4 the representation effect is larger, and from MACCS neither effect is significantly larger. On the classification datasets, only one main factorial design has a significant difference between the two effects. Although the model effect is smaller on solubility and lipophilicity, TabFM outperforms the RF on all 7 datasets when both use RDKit descriptors. With RDKit descriptors in place of a fingerprint, the RF baseline reported for DGT surpasses the transformer's published solubility score. We recommend that model comparisons evaluate classical baselines on more than one representation and report the representation and model effects separately.

==> generated/dgt_seeds.tex <==
\newcommand{\DgtSeedN}{4}
\newcommand{\DgtSeedSigBbbp}{2}
\newcommand{\DgtBbbpWinningSeeds}{0 and 3}


==> generated/external_similarity.tex <==
\newcommand{\ExtSimEsol}{0.38}
\newcommand{\ExtSimEsolMN}{0.42}
\newcommand{\ExtSimLipo}{0.29}
\newcommand{\ExtSimLipoMN}{0.54}


==> generated/timing.tex <==
\newcommand{\TimeGpuMem}{40}
\newcommand{\TimeCpus}{12}
\newcommand{\TimeFmRam}{13}
\newcommand{\TimeFmGpuMax}{17}
\newcommand{\TimeNEsol}{1,128}
\newcommand{\TimeNLipo}{4,200}
\newcommand{\TimeSiderTasks}{27}
\newcommand{\TimeClintoxTasks}{2}
\newcommand{\TimeFmRamMeasured}{13.1}
\newcommand{\TimeFmGpuEsol}{8.9}
\newcommand{\TimeFmGpuLipo}{17.1}
\newcommand{\TimePfnRfLo}{0.5}
\newcommand{\TimePfnRfHi}{0.6}
\newcommand{\TimeFmRfLo}{1.8}
\newcommand{\TimeFmRfHi}{1.9}
\newcommand{\TimeFmRamTimes}{30}

